Dynamic cache reconfiguration based techniques for improving cache energy efficiency

Modern multicore processors are employing large last-level caches, for example Intel's E7-8800 processor uses 24MB L3 cache. Further, with each CMOS technology generation, leakage energy has been dramatically increasing and hence, leakage energy is expected to become a major source of energy dissipation, especially in last-level caches (LLCs). The conventional schemes of cache energy saving either aim at saving dynamic energy or are based on properties specific to first-level caches, and thus these schemes have limited utility for last-level caches. Further, several other techniques require offline profiling or per-application tuning and hence are not suitable for product systems. In this research, we propose novel cache leakage energy saving schemes for single-core and multicore systems; desktop, QoS, real-time and server systems. We propose software-controlled, hardware-assisted techniques which use dynamic cache reconfiguration to configure the cache to the most energy efficient configuration while keeping the performance loss bounded. To profile and test a large number of potential configurations, we utilize low-overhead, micro-architecture components, which can be easily integrated into modern processor chips. We adopt a system-wide approach to save energy to ensure that cache reconfiguration does not increase energy consumption of other components of the processor. We have compared our techniques with the state-of-art techniques and have found that our techniques outperform them in their energy efficiency. This research has important applications in improving energy-efficiency of higher-end embedded, desktop, server processors and multitasking systems. We have also proposed performance estimation approach for efficient design space exploration and have implemented time-sampling based simulation acceleration approach for full-system architectural simulators.

==> log1 <==
latex SparshMittal_PhD_Thesis
This is pdfeTeX, Version 3.141592-1.21a-2.2 (Web2C 7.5.4)
entering extended mode
(./SparshMittal_PhD_Thesis.tex
LaTeX2e <2003/12/01>
Babel <v3.8d> and hyphenation patterns for american, french, german, ngerman, b
ahasa, basque, bulgarian, catalan, croatian, czech, danish, dutch, esperanto, e
stonian, finnish, greek, icelandic, irish, italian, latin, magyar, norsk, polis
h, portuges, romanian, russian, serbian, slovak, slovene, spanish, swedish, tur
kish, ukrainian, nohyphenation, loaded.
(./isuthesis.cls
Document Class: isuthesis 2011/02/14 v1.03 (Joe Struss)
Document Class: isuthesis 2011/02/14
(/usr/share/texmf/tex/latex/base/report.cls
Document Class: report 2004/02/16 v1.4f Standard LaTeX document class
(/usr/share/texmf/tex/latex/base/size11.clo))
(/usr/share/texmf/tex/latex/geometry/geometry.sty
(/usr/share/texmf/tex/latex/graphics/keyval.sty)
(/usr/share/texmf/tex/latex/geometry/geometry.cfg))) (./flushend.sty)
(/usr/share/texmf/tex/latex/preprint/fullpage.sty)
(/usr/share/texmf/tex/latex/float/float.sty)
(/usr/share/texmf/tex/latex/graphics/graphicx.sty
(/usr/share/texmf/tex/latex/graphics/graphics.sty
(/usr/share/texmf/tex/latex/graphics/trig.sty)
(/usr/share/texmf/tex/latex/graphics/graphics.cfg)
(/usr/share/texmf/tex/latex/graphics/dvips.def)))
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty)
(/usr/share/texmf/tex/latex/graphics/color.sty
(/usr/share/texmf/tex/latex/graphics/color.cfg)
(/usr/share/texmf/tex/latex/graphics/dvipsnam.def)) (./algorithmic.sty
Document Style `algorithmic' - environment
(/usr/share/texmf/tex/latex/base/ifthen.sty)
(/usr/share/texmf/tex/latex/tools/calc.sty)) (./algorithm.sty
Document Style `algorithm' - floating environment
) (/usr/share/texmf/tex/latex/multirow/multirow.sty)
(/usr/share/texmf/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/share/texmf/tex/latex/subfigure/subfigure.cfg))
(/usr/share/texmf/tex/latex/url/url.sty)
(/usr/share/texmf/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf/tex/latex/amsmath/amstext.sty
(/usr/share/texmf/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf/tex/latex/amsmath/amsopn.sty)) (./isutraditional.sty)
(./rotating.sty) (./natbib.sty)
(/usr/share/texmf/tex/latex/multibib/multibib.sty) (./refpaper.aux)
(/usr/share/texmf/tex/latex/cite/chapterbib.sty)
(/usr/share/texmf/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf/tex/latex/hyperref/hyperref.cfg)
Implicit mode ON; LaTeX internals redefined
)
*hyperref using default driver hdvips*
(/usr/share/texmf/tex/latex/hyperref/hdvips.def
(/usr/share/texmf/tex/latex/hyperref/pdfmark.def))
(./SparshMittal_PhD_Thesis.aux (./work_common/titlepage.aux)
(./work_common/dedication.aux) (./work_common/acknowl.aux)
(./work_common/abstract.aux) (./work_common/introduction.aux)
(./work_common/contributions.aux) (./work_common/relatedwork.aux)
(./work_esto/work_esto.aux) (./work_encache/work_encache.aux)
(./work_palette/work_palette.aux) (./work_cashier/work_cashier.aux)
(./work_master/work_master.aux) (./work_manager/work_manager.aux)
(./work_simulation/work_simulation.aux) (./work_common/work_publications.aux))
(/usr/share/texmf/tex/latex/hyperref/nameref.sty)
(./SparshMittal_PhD_Thesis.out) (./SparshMittal_PhD_Thesis.out)
(./work_common/titlepage.tex) (/usr/share/texmf/tex/latex/base/omscmr.fd)
Overfull \vbox (5.43898pt too high) detected at line 65
[1] (./work_common/dedication.tex)
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[2] (./SparshMittal_PhD_Thesis.toc (/usr/share/texmf/tex/latex/amsfonts/umsa.fd
) (/usr/share/texmf/tex/latex/amsfonts/umsb.fd)
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[3] [4] [5] [6]) [7] (./SparshMittal_PhD_Thesis.lot)
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[8] (./SparshMittal_PhD_Thesis.lof
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[9]) [10] (./work_common/acknowl.tex
ACKNOWLEDGEMENTS
) [11] (./work_common/abstract.tex
ABSTRACT
) [12] (./work_common/introduction.tex
CHAPTER\  1.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[1] [2] [3]) [4] (./work_common/contributions.tex
CHAPTER\  2.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[5] [6]) [7] (./work_common/relatedwork.tex
CHAPTER\  3.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[8] [9] [10]) [11] (./work_esto/work_esto.tex
CHAPTER\  4.
(./work_esto/intro.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[12] [13]) (./work_esto/motivation.tex [14]) (./work_esto/methods.tex
<work_esto/ESTOflow.eps> [15] [16] [17]
Overfull \hbox (13.41255pt too wide) in paragraph at lines 55--74
[]\OT1/cmr/m/n/10.95 Here, for any con-fig-u-ra-tion, we have cor-re-spond-ing 
$\OML/cmm/m/it/10.95 M[]$\OT1/cmr/m/n/10.95 =L2 misses, $\OML/cmm/m/it/10.95 H[
]$\OT1/cmr/m/n/10.95 =L2 hits, $\OML/cmm/m/it/10.95 Time$\OT1/cmr/m/n/10.95 =ex
ecution
<work_esto/ErrorTime.eps> <work_esto/ErrorEnergy.eps>
Overfull \hbox (5.7795pt too wide) in paragraph at lines 89--93
 [] 

Overfull \hbox (5.7795pt too wide) in paragraph at lines 89--93
 [][] 
[18] [19]) (./work_esto/results.tex [20] [21] <work_esto/ErrorTimeSize.eps>
<work_esto/ErrorEnergySize.eps>) (./work_esto/background.tex [22] [23])
(./work_esto/conclusion.tex)) [24] (./work_encache/work_encache.tex
CHAPTER\  5.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[25] <work_encache/encache_ProfileCacheFlowDiag.eps> [26]
<work_encache/Prof2.eps> <work_encache/Prof4.eps> <work_encache/Prof8.eps>
[27] [28] <work_encache/EnCache_L2Diagram.eps> [29] [30] [31]
<work_encache/EDP2.eps> <work_encache/Energy2.eps> <work_encache/Cycle2.eps>
<work_encache/EDP4.eps> <work_encache/Energy4.eps> <work_encache/Cycle4.eps>
<work_encache/EDP8.eps> <work_encache/Energy8.eps> <work_encache/Cycle8.eps>
[32] [33] [34] [35]) [36] (./work_palette/work_palette.tex
CHAPTER\  6.
(./work_palette/intro1.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[37]) (./work_palette/motivation1.tex) (./work_palette/background1.tex [38]
[39]) (./work_palette/method1.tex <work_palette/Figures/Overalldiagram.eps>
[40] [41] <work_palette/Figures/RCEdiagram1.eps> [42] [43])
(./work_palette/energysavingalgorithm.tex [44] [45])
(./work_palette/implementation.tex [46])
(./work_palette/experimental_platform1.tex [47] [48] [49])
(./work_palette/results1.tex <work_palette/Figures/Energy2M.eps>
<work_palette/Figures/Time2M.eps> [50] <work_palette/Figures/EDP2M.eps>
<work_palette/Figures/AR2M.eps> <work_palette/Figures/Miss2M.eps> [51] [52])
(./work_palette/results2.tex) (./work_palette/conclusion1.tex)) [53]
(./work_cashier/work_cashier.tex
CHAPTER\  7.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[54] <work_cashier/Cashier_RemappingFigure.eps> [55] [56] [57] [58] [59]
[60] <work_cashier/MSM_Energy_2M.eps> <work_cashier/MSM_Time_2M.eps>
Overfull \hbox (5.7795pt too wide) in paragraph at lines 124--126
 [][] 

Overfull \hbox (5.7795pt too wide) in paragraph at lines 124--126
 [] 
[61] [62]) [63] (./work_master/work_master.tex
CHAPTER\  8.
(./work_master/intro.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[64] [65]) (./work_master/background.tex
<work_master/Figures/BlockDiagram.eps> [66]) (./work_master/method.tex [67]
[68] [69] <work_master/Figures/RCEdesign.eps> [70] [71])
(./work_master/energysavingalgo.tex [72] [73])
(./work_master/hardware_implementation.tex [74] [75])
(./work_master/experimentalmethodology.tex [76] [77] [78]
<work_master/Figures/C2MB4_Energy.eps> <work_master/Figures/C2MB4_WIPC.eps>
[79] [80]) (./work_master/results.tex [81]
<work_master/Figures/C4MB8_Energy.eps> <work_master/Figures/C4MB8_WIPC.eps>
[82] [83]) (./work_master/results2.tex [84]) (./work_master/conclusion.tex
[85])) [86] (./work_manager/work_manager.tex
CHAPTER\  9.
(./work_manager/q_intro.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[87]) (./work_manager/q_methods.tex [88]
<work_manager/Figures/FlowDiagram1.eps> [89] [90]
<work_manager/Figures/RCEdiagram.eps> [91] [92])
(./work_manager/q_energysavingalgorithm.tex [93] [94])
(./work_manager/q_implementation.tex [95])
(./work_manager/q_experimentalplatform.tex [96])
(./work_manager/q_energymodel.tex <work_manager/Figures/C2MB4_Energy.eps>
<work_manager/Figures/C2MB4_AR.eps> <work_manager/Figures/C2MB4_WIPC.eps>
[97] [98]) (./work_manager/q_results.tex [99] [100])
(./work_manager/q_background.tex)) [101] (./work_simulation/work_simulation.tex

CHAPTER\  10.

Package hyperref Warning: Difference (2) between bookmark levels is greater 
(hyperref)                than one, level fixed on input line 4.

<work_simulation/simulation_BlockDiagramMain.eps>
Overfull \hbox (20.46898pt too wide) in paragraph at lines 10--11
 [][] 

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[102] [103] [104] [105] [106] [107] <work_simulation/CPIValueFinal.eps>
<work_simulation/CPIErrorFinal.eps>
Overfull \hbox (27.4011pt too wide) in paragraph at lines 75--77
 [] 

Overfull \hbox (29.23297pt too wide) in paragraph at lines 75--77
 [][] 
[108] [109]) [110] (./work_common/work_publications.tex
CHAPTER\  11.

LaTeX Warning: Citation `MitZha13_Cashier' in file `work_common/work_publicatio
ns' undefined on input line 15.


LaTeX Warning: Citation `Mit2013_DesignContest' in file `work_common/work_publi
cations' undefined on input line 16.


LaTeX Warning: Citation `MitZha12_Simulation' in file `work_common/work_publica
tions' undefined on input line 17.


LaTeX Warning: Citation `MitZha12_EnCache' in file `work_common/work_publicatio
ns' undefined on input line 18.


LaTeX Warning: Citation `mittal_simplex' in file `work_common/work_publications
' undefined on input line 19.


LaTeX Warning: Citation `mittal_fpga' in file `work_common/work_publications' u
ndefined on input line 20.


LaTeX Warning: Citation `mittal_sysgen' in file `work_common/work_publications'
 undefined on input line 21.


LaTeX Warning: Citation `gupta_guaranteed' in file `work_common/work_publicatio
ns' undefined on input line 22.


LaTeX Warning: Citation `GupMit08_MIMO' in file `work_common/work_publications'
 undefined on input line 23.


LaTeX Warning: Citation `MitGup08_BioinQA' in file `work_common/work_publicatio
ns' undefined on input line 24.


LaTeX Warning: Citation `gupta_eureqa' in file `work_common/work_publications' 
undefined on input line 25.


LaTeX Warning: Citation `mittal_caffet' in file `work_common/work_publications'
 undefined on input line 26.

No file work_common/work_publications.bbl.
)
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[111] (./SparshMittal_PhD_Thesis.bbl
Overfull \hbox (9.0pt too wide) in paragraph at lines 1--1
 []   [] 

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[112] [113] [114] [115] [116] [117] [118] [119]
Underfull \hbox (badness 4673) in paragraph at lines 497--501
[]\OT1/cmr/m/n/10.95 M. Monchiero et al.  De-sign space ex-plo-ration for mul-t
i-core ar-chi-tec-tures: a
[120] [121] [122] [123] [124] [125]) [126] (./SparshMittal_PhD_Thesis.aux
(./work_common/titlepage.aux) (./work_common/dedication.aux)
(./work_common/acknowl.aux) (./work_common/abstract.aux)
(./work_common/introduction.aux) (./work_common/contributions.aux)
(./work_common/relatedwork.aux) (./work_esto/work_esto.aux)
(./work_encache/work_encache.aux) (./work_palette/work_palette.aux)
(./work_cashier/work_cashier.aux) (./work_master/work_master.aux)
(./work_manager/work_manager.aux) (./work_simulation/work_simulation.aux)
(./work_common/work_publications.aux))

LaTeX Warning: There were undefined references.

 )
(see the transcript file for additional information)
Output written on SparshMittal_PhD_Thesis.dvi (138 pages, 611056 bytes).
Transcript written on SparshMittal_PhD_Thesis.log.
bibtex -min-crossrefs=99 SparshMittal_PhD_Thesis
This is BibTeX, Version 0.99c (Web2C 7.5.4)
The top-level auxiliary file: SparshMittal_PhD_Thesis.aux
A level-1 auxiliary file: work_common/titlepage.aux
A level-1 auxiliary file: work_common/dedication.aux
A level-1 auxiliary file: work_common/acknowl.aux
A level-1 auxiliary file: work_common/abstract.aux
A level-1 auxiliary file: work_common/introduction.aux
A level-1 auxiliary file: work_common/contributions.aux
A level-1 auxiliary file: work_common/relatedwork.aux
A level-1 auxiliary file: work_esto/work_esto.aux
A level-1 auxiliary file: work_encache/work_encache.aux
A level-1 auxiliary file: work_palette/work_palette.aux
A level-1 auxiliary file: work_cashier/work_cashier.aux
A level-1 auxiliary file: work_master/work_master.aux
A level-1 auxiliary file: work_manager/work_manager.aux
A level-1 auxiliary file: work_simulation/work_simulation.aux
A level-1 auxiliary file: work_common/work_publications.aux
The style file: plain.bst
Database file #1: PhDReferences.bib
Warning--to sort, need author or key in top500list
Warning--to sort, need author or key in semiconductor2011international
Warning--to sort, need author or key in random
Warning--to sort, need author or key in gemstutorial
Warning--can't use both volume and number fields in chou2004microarchitecture
Warning--empty booktitle in LiKad02_LeakageEnergy
Warning--can't use both volume and number fields in nesbit2007virtual
Warning--can't use both volume and number fields in wenisch2005turbosmarts
(There were 8 warnings)
bibtex -min-crossrefs=99 refpaper	
This is BibTeX, Version 0.99c (Web2C 7.5.4)
The top-level auxiliary file: refpaper.aux
The style file: plain.bst
Database file #1: PhDReferences.bib
Warning--I didn't find a database entry for "mittal_simplex"
Warning--I didn't find a database entry for "mittal_fpga"
Warning--I didn't find a database entry for "mittal_sysgen"
Warning--I didn't find a database entry for "gupta_guaranteed"
Warning--I didn't find a database entry for "gupta_eureqa"
Warning--I didn't find a database entry for "mittal_caffet"
(There were 6 warnings)
latex SparshMittal_PhD_Thesis
This is pdfeTeX, Version 3.141592-1.21a-2.2 (Web2C 7.5.4)
entering extended mode
(./SparshMittal_PhD_Thesis.tex
LaTeX2e <2003/12/01>
Babel <v3.8d> and hyphenation patterns for american, french, german, ngerman, b
ahasa, basque, bulgarian, catalan, croatian, czech, danish, dutch, esperanto, e
stonian, finnish, greek, icelandic, irish, italian, latin, magyar, norsk, polis
h, portuges, romanian, russian, serbian, slovak, slovene, spanish, swedish, tur
kish, ukrainian, nohyphenation, loaded.
(./isuthesis.cls
Document Class: isuthesis 2011/02/14 v1.03 (Joe Struss)
Document Class: isuthesis 2011/02/14
(/usr/share/texmf/tex/latex/base/report.cls
Document Class: report 2004/02/16 v1.4f Standard LaTeX document class
(/usr/share/texmf/tex/latex/base/size11.clo))
(/usr/share/texmf/tex/latex/geometry/geometry.sty
(/usr/share/texmf/tex/latex/graphics/keyval.sty)
(/usr/share/texmf/tex/latex/geometry/geometry.cfg))) (./flushend.sty)
(/usr/share/texmf/tex/latex/preprint/fullpage.sty)
(/usr/share/texmf/tex/latex/float/float.sty)
(/usr/share/texmf/tex/latex/graphics/graphicx.sty
(/usr/share/texmf/tex/latex/graphics/graphics.sty
(/usr/share/texmf/tex/latex/graphics/trig.sty)
(/usr/share/texmf/tex/latex/graphics/graphics.cfg)
(/usr/share/texmf/tex/latex/graphics/dvips.def)))
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty)
(/usr/share/texmf/tex/latex/graphics/color.sty
(/usr/share/texmf/tex/latex/graphics/color.cfg)
(/usr/share/texmf/tex/latex/graphics/dvipsnam.def)) (./algorithmic.sty
Document Style `algorithmic' - environment
(/usr/share/texmf/tex/latex/base/ifthen.sty)
(/usr/share/texmf/tex/latex/tools/calc.sty)) (./algorithm.sty
Document Style `algorithm' - floating environment
) (/usr/share/texmf/tex/latex/multirow/multirow.sty)
(/usr/share/texmf/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/share/texmf/tex/latex/subfigure/subfigure.cfg))
(/usr/share/texmf/tex/latex/url/url.sty)
(/usr/share/texmf/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf/tex/latex/amsmath/amstext.sty
(/usr/share/texmf/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf/tex/latex/amsmath/amsopn.sty)) (./isutraditional.sty)
(./rotating.sty) (./natbib.sty)
(/usr/share/texmf/tex/latex/multibib/multibib.sty) (./refpaper.aux)
(/usr/share/texmf/tex/latex/cite/chapterbib.sty)
(/usr/share/texmf/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf/tex/latex/hyperref/hyperref.cfg)
Implicit mode ON; LaTeX internals redefined
)
*hyperref using default driver hdvips*
(/usr/share/texmf/tex/latex/hyperref/hdvips.def
(/usr/share/texmf/tex/latex/hyperref/pdfmark.def))
(./SparshMittal_PhD_Thesis.aux (./work_common/titlepage.aux)
(./work_common/dedication.aux) (./work_common/acknowl.aux)
(./work_common/abstract.aux) (./work_common/introduction.aux)
(./work_common/contributions.aux) (./work_common/relatedwork.aux)
(./work_esto/work_esto.aux) (./work_encache/work_encache.aux)
(./work_palette/work_palette.aux) (./work_cashier/work_cashier.aux)
(./work_master/work_master.aux) (./work_manager/work_manager.aux)
(./work_simulation/work_simulation.aux) (./work_common/work_publications.aux))
(/usr/share/texmf/tex/latex/hyperref/nameref.sty)
(./SparshMittal_PhD_Thesis.out) (./SparshMittal_PhD_Thesis.out)
(./work_common/titlepage.tex) (/usr/share/texmf/tex/latex/base/omscmr.fd)
Overfull \vbox (5.43898pt too high) detected at line 65
[1] (./work_common/dedication.tex)
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[2] (./SparshMittal_PhD_Thesis.toc (/usr/share/texmf/tex/latex/amsfonts/umsa.fd
) (/usr/share/texmf/tex/latex/amsfonts/umsb.fd)
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[3] [4] [5] [6]) [7] (./SparshMittal_PhD_Thesis.lot)
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[8] (./SparshMittal_PhD_Thesis.lof
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[9]) [10] (./work_common/acknowl.tex
ACKNOWLEDGEMENTS
) [11] (./work_common/abstract.tex
ABSTRACT
) [12] (./work_common/introduction.tex
CHAPTER\  1.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[1] [2] [3]) [4] (./work_common/contributions.tex
CHAPTER\  2.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[5] [6]) [7] (./work_common/relatedwork.tex
CHAPTER\  3.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[8] [9] [10]) [11] (./work_esto/work_esto.tex
CHAPTER\  4.
(./work_esto/intro.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[12] [13]) (./work_esto/motivation.tex [14]) (./work_esto/methods.tex
<work_esto/ESTOflow.eps> [15] [16] [17]
Overfull \hbox (13.41255pt too wide) in paragraph at lines 55--74
[]\OT1/cmr/m/n/10.95 Here, for any con-fig-u-ra-tion, we have cor-re-spond-ing 
$\OML/cmm/m/it/10.95 M[]$\OT1/cmr/m/n/10.95 =L2 misses, $\OML/cmm/m/it/10.95 H[
]$\OT1/cmr/m/n/10.95 =L2 hits, $\OML/cmm/m/it/10.95 Time$\OT1/cmr/m/n/10.95 =ex
ecution
<work_esto/ErrorTime.eps> <work_esto/ErrorEnergy.eps>
Overfull \hbox (5.7795pt too wide) in paragraph at lines 89--93
 [] 

Overfull \hbox (5.7795pt too wide) in paragraph at lines 89--93
 [][] 
[18] [19]) (./work_esto/results.tex [20] [21] <work_esto/ErrorTimeSize.eps>
<work_esto/ErrorEnergySize.eps>) (./work_esto/background.tex [22] [23])
(./work_esto/conclusion.tex)) [24] (./work_encache/work_encache.tex
CHAPTER\  5.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[25] <work_encache/encache_ProfileCacheFlowDiag.eps> [26]
<work_encache/Prof2.eps> <work_encache/Prof4.eps> <work_encache/Prof8.eps>
[27] [28] <work_encache/EnCache_L2Diagram.eps> [29] [30] [31]
<work_encache/EDP2.eps> <work_encache/Energy2.eps> <work_encache/Cycle2.eps>
<work_encache/EDP4.eps> <work_encache/Energy4.eps> <work_encache/Cycle4.eps>
<work_encache/EDP8.eps> <work_encache/Energy8.eps> <work_encache/Cycle8.eps>
[32] [33] [34] [35]) [36] (./work_palette/work_palette.tex
CHAPTER\  6.
(./work_palette/intro1.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[37]) (./work_palette/motivation1.tex) (./work_palette/background1.tex [38]
[39]) (./work_palette/method1.tex <work_palette/Figures/Overalldiagram.eps>
[40] [41] <work_palette/Figures/RCEdiagram1.eps> [42] [43])
(./work_palette/energysavingalgorithm.tex [44] [45])
(./work_palette/implementation.tex [46])
(./work_palette/experimental_platform1.tex [47] [48] [49])
(./work_palette/results1.tex <work_palette/Figures/Energy2M.eps>
<work_palette/Figures/Time2M.eps> [50] <work_palette/Figures/EDP2M.eps>
<work_palette/Figures/AR2M.eps> <work_palette/Figures/Miss2M.eps> [51] [52])
(./work_palette/results2.tex) (./work_palette/conclusion1.tex)) [53]
(./work_cashier/work_cashier.tex
CHAPTER\  7.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[54] <work_cashier/Cashier_RemappingFigure.eps> [55] [56] [57] [58] [59]
[60] <work_cashier/MSM_Energy_2M.eps> <work_cashier/MSM_Time_2M.eps>
Overfull \hbox (5.7795pt too wide) in paragraph at lines 124--126
 [][] 

Overfull \hbox (5.7795pt too wide) in paragraph at lines 124--126
 [] 
[61] [62]) [63] (./work_master/work_master.tex
CHAPTER\  8.
(./work_master/intro.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[64] [65]) (./work_master/background.tex
<work_master/Figures/BlockDiagram.eps> [66]) (./work_master/method.tex [67]
[68] [69] <work_master/Figures/RCEdesign.eps> [70] [71])
(./work_master/energysavingalgo.tex [72] [73])
(./work_master/hardware_implementation.tex [74] [75])
(./work_master/experimentalmethodology.tex [76] [77] [78]
<work_master/Figures/C2MB4_Energy.eps> <work_master/Figures/C2MB4_WIPC.eps>
[79] [80]) (./work_master/results.tex [81]
<work_master/Figures/C4MB8_Energy.eps> <work_master/Figures/C4MB8_WIPC.eps>
[82] [83]) (./work_master/results2.tex [84]) (./work_master/conclusion.tex
[85])) [86] (./work_manager/work_manager.tex
CHAPTER\  9.
(./work_manager/q_intro.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[87]) (./work_manager/q_methods.tex [88]
<work_manager/Figures/FlowDiagram1.eps> [89] [90]
<work_manager/Figures/RCEdiagram.eps> [91] [92])
(./work_manager/q_energysavingalgorithm.tex [93] [94])
(./work_manager/q_implementation.tex [95])
(./work_manager/q_experimentalplatform.tex [96])
(./work_manager/q_energymodel.tex <work_manager/Figures/C2MB4_Energy.eps>
<work_manager/Figures/C2MB4_AR.eps> <work_manager/Figures/C2MB4_WIPC.eps>
[97] [98]) (./work_manager/q_results.tex [99] [100])
(./work_manager/q_background.tex)) [101] (./work_simulation/work_simulation.tex

CHAPTER\  10.

Package hyperref Warning: Difference (2) between bookmark levels is greater 
(hyperref)                than one, level fixed on input line 4.

<work_simulation/simulation_BlockDiagramMain.eps>
Overfull \hbox (20.46898pt too wide) in paragraph at lines 10--11
 [][] 

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[102] [103] [104] [105] [106] [107] <work_simulation/CPIValueFinal.eps>
<work_simulation/CPIErrorFinal.eps>
Overfull \hbox (27.4011pt too wide) in paragraph at lines 75--77
 [] 

Overfull \hbox (29.23297pt too wide) in paragraph at lines 75--77
 [][] 
[108] [109]) [110] (./work_common/work_publications.tex
CHAPTER\  11.

LaTeX Warning: Citation `MitZha13_Cashier' in file `work_common/work_publicatio
ns' undefined on input line 15.


LaTeX Warning: Citation `Mit2013_DesignContest' in file `work_common/work_publi
cations' undefined on input line 16.


LaTeX Warning: Citation `MitZha12_Simulation' in file `work_common/work_publica
tions' undefined on input line 17.


LaTeX Warning: Citation `MitZha12_EnCache' in file `work_common/work_publicatio
ns' undefined on input line 18.


LaTeX Warning: Citation `mittal_simplex' in file `work_common/work_publications
' undefined on input line 19.


LaTeX Warning: Citation `mittal_fpga' in file `work_common/work_publications' u
ndefined on input line 20.


LaTeX Warning: Citation `mittal_sysgen' in file `work_common/work_publications'
 undefined on input line 21.


LaTeX Warning: Citation `gupta_guaranteed' in file `work_common/work_publicatio
ns' undefined on input line 22.


LaTeX Warning: Citation `GupMit08_MIMO' in file `work_common/work_publications'
 undefined on input line 23.


LaTeX Warning: Citation `MitGup08_BioinQA' in file `work_common/work_publicatio
ns' undefined on input line 24.


LaTeX Warning: Citation `gupta_eureqa' in file `work_common/work_publications' 
undefined on input line 25.


LaTeX Warning: Citation `mittal_caffet' in file `work_common/work_publications'
 undefined on input line 26.

No file work_common/work_publications.bbl.
)
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[111] (./SparshMittal_PhD_Thesis.bbl
Overfull \hbox (9.0pt too wide) in paragraph at lines 1--1
 []   [] 

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[112] [113] [114] [115] [116] [117] [118] [119]
Underfull \hbox (badness 4673) in paragraph at lines 497--501
[]\OT1/cmr/m/n/10.95 M. Monchiero et al.  De-sign space ex-plo-ration for mul-t
i-core ar-chi-tec-tures: a
[120] [121] [122] [123] [124] [125]) [126] (./SparshMittal_PhD_Thesis.aux
(./work_common/titlepage.aux) (./work_common/dedication.aux)
(./work_common/acknowl.aux) (./work_common/abstract.aux)
(./work_common/introduction.aux) (./work_common/contributions.aux)
(./work_common/relatedwork.aux) (./work_esto/work_esto.aux)
(./work_encache/work_encache.aux) (./work_palette/work_palette.aux)
(./work_cashier/work_cashier.aux) (./work_master/work_master.aux)
(./work_manager/work_manager.aux) (./work_simulation/work_simulation.aux)
(./work_common/work_publications.aux))

LaTeX Warning: There were undefined references.

 )
(see the transcript file for additional information)
Output written on SparshMittal_PhD_Thesis.dvi (138 pages, 611056 bytes).
Transcript written on SparshMittal_PhD_Thesis.log.
latex SparshMittal_PhD_Thesis
This is pdfeTeX, Version 3.141592-1.21a-2.2 (Web2C 7.5.4)
entering extended mode
(./SparshMittal_PhD_Thesis.tex
LaTeX2e <2003/12/01>
Babel <v3.8d> and hyphenation patterns for american, french, german, ngerman, b
ahasa, basque, bulgarian, catalan, croatian, czech, danish, dutch, esperanto, e
stonian, finnish, greek, icelandic, irish, italian, latin, magyar, norsk, polis
h, portuges, romanian, russian, serbian, slovak, slovene, spanish, swedish, tur
kish, ukrainian, nohyphenation, loaded.
(./isuthesis.cls
Document Class: isuthesis 2011/02/14 v1.03 (Joe Struss)
Document Class: isuthesis 2011/02/14
(/usr/share/texmf/tex/latex/base/report.cls
Document Class: report 2004/02/16 v1.4f Standard LaTeX document class
(/usr/share/texmf/tex/latex/base/size11.clo))
(/usr/share/texmf/tex/latex/geometry/geometry.sty
(/usr/share/texmf/tex/latex/graphics/keyval.sty)
(/usr/share/texmf/tex/latex/geometry/geometry.cfg))) (./flushend.sty)
(/usr/share/texmf/tex/latex/preprint/fullpage.sty)
(/usr/share/texmf/tex/latex/float/float.sty)
(/usr/share/texmf/tex/latex/graphics/graphicx.sty
(/usr/share/texmf/tex/latex/graphics/graphics.sty
(/usr/share/texmf/tex/latex/graphics/trig.sty)
(/usr/share/texmf/tex/latex/graphics/graphics.cfg)
(/usr/share/texmf/tex/latex/graphics/dvips.def)))
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty)
(/usr/share/texmf/tex/latex/graphics/color.sty
(/usr/share/texmf/tex/latex/graphics/color.cfg)
(/usr/share/texmf/tex/latex/graphics/dvipsnam.def)) (./algorithmic.sty
Document Style `algorithmic' - environment
(/usr/share/texmf/tex/latex/base/ifthen.sty)
(/usr/share/texmf/tex/latex/tools/calc.sty)) (./algorithm.sty
Document Style `algorithm' - floating environment
) (/usr/share/texmf/tex/latex/multirow/multirow.sty)
(/usr/share/texmf/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/share/texmf/tex/latex/subfigure/subfigure.cfg))
(/usr/share/texmf/tex/latex/url/url.sty)
(/usr/share/texmf/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf/tex/latex/amsmath/amstext.sty
(/usr/share/texmf/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf/tex/latex/amsmath/amsopn.sty)) (./isutraditional.sty)
(./rotating.sty) (./natbib.sty)
(/usr/share/texmf/tex/latex/multibib/multibib.sty) (./refpaper.aux)
(/usr/share/texmf/tex/latex/cite/chapterbib.sty)
(/usr/share/texmf/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf/tex/latex/hyperref/hyperref.cfg)
Implicit mode ON; LaTeX internals redefined
)
*hyperref using default driver hdvips*
(/usr/share/texmf/tex/latex/hyperref/hdvips.def
(/usr/share/texmf/tex/latex/hyperref/pdfmark.def))
(./SparshMittal_PhD_Thesis.aux (./work_common/titlepage.aux)
(./work_common/dedication.aux) (./work_common/acknowl.aux)
(./work_common/abstract.aux) (./work_common/introduction.aux)
(./work_common/contributions.aux) (./work_common/relatedwork.aux)
(./work_esto/work_esto.aux) (./work_encache/work_encache.aux)
(./work_palette/work_palette.aux) (./work_cashier/work_cashier.aux)
(./work_master/work_master.aux) (./work_manager/work_manager.aux)
(./work_simulation/work_simulation.aux) (./work_common/work_publications.aux))
(/usr/share/texmf/tex/latex/hyperref/nameref.sty)
(./SparshMittal_PhD_Thesis.out) (./SparshMittal_PhD_Thesis.out)
(./work_common/titlepage.tex) (/usr/share/texmf/tex/latex/base/omscmr.fd)
Overfull \vbox (5.43898pt too high) detected at line 65
[1] (./work_common/dedication.tex)
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[2] (./SparshMittal_PhD_Thesis.toc (/usr/share/texmf/tex/latex/amsfonts/umsa.fd
) (/usr/share/texmf/tex/latex/amsfonts/umsb.fd)
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[3] [4] [5] [6]) [7] (./SparshMittal_PhD_Thesis.lot)
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[8] (./SparshMittal_PhD_Thesis.lof
Overfull \vbox (7.31305pt too high) has occurred while \output is active
[9]) [10] (./work_common/acknowl.tex
ACKNOWLEDGEMENTS
) [11] (./work_common/abstract.tex
ABSTRACT
) [12] (./work_common/introduction.tex
CHAPTER\  1.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[1] [2] [3]) [4] (./work_common/contributions.tex
CHAPTER\  2.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[5] [6]) [7] (./work_common/relatedwork.tex
CHAPTER\  3.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[8] [9] [10]) [11] (./work_esto/work_esto.tex
CHAPTER\  4.
(./work_esto/intro.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[12] [13]) (./work_esto/motivation.tex [14]) (./work_esto/methods.tex
<work_esto/ESTOflow.eps> [15] [16] [17]
Overfull \hbox (13.41255pt too wide) in paragraph at lines 55--74
[]\OT1/cmr/m/n/10.95 Here, for any con-fig-u-ra-tion, we have cor-re-spond-ing 
$\OML/cmm/m/it/10.95 M[]$\OT1/cmr/m/n/10.95 =L2 misses, $\OML/cmm/m/it/10.95 H[
]$\OT1/cmr/m/n/10.95 =L2 hits, $\OML/cmm/m/it/10.95 Time$\OT1/cmr/m/n/10.95 =ex
ecution
<work_esto/ErrorTime.eps> <work_esto/ErrorEnergy.eps>
Overfull \hbox (5.7795pt too wide) in paragraph at lines 89--93
 [] 

Overfull \hbox (5.7795pt too wide) in paragraph at lines 89--93
 [][] 
[18] [19]) (./work_esto/results.tex [20] [21] <work_esto/ErrorTimeSize.eps>
<work_esto/ErrorEnergySize.eps>) (./work_esto/background.tex [22] [23])
(./work_esto/conclusion.tex)) [24] (./work_encache/work_encache.tex
CHAPTER\  5.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[25] <work_encache/encache_ProfileCacheFlowDiag.eps> [26]
<work_encache/Prof2.eps> <work_encache/Prof4.eps> <work_encache/Prof8.eps>
[27] [28] <work_encache/EnCache_L2Diagram.eps> [29] [30] [31]
<work_encache/EDP2.eps> <work_encache/Energy2.eps> <work_encache/Cycle2.eps>
<work_encache/EDP4.eps> <work_encache/Energy4.eps> <work_encache/Cycle4.eps>
<work_encache/EDP8.eps> <work_encache/Energy8.eps> <work_encache/Cycle8.eps>
[32] [33] [34] [35]) [36] (./work_palette/work_palette.tex
CHAPTER\  6.
(./work_palette/intro1.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[37]) (./work_palette/motivation1.tex) (./work_palette/background1.tex [38]
[39]) (./work_palette/method1.tex <work_palette/Figures/Overalldiagram.eps>
[40] [41] <work_palette/Figures/RCEdiagram1.eps> [42] [43])
(./work_palette/energysavingalgorithm.tex [44] [45])
(./work_palette/implementation.tex [46])
(./work_palette/experimental_platform1.tex [47] [48] [49])
(./work_palette/results1.tex <work_palette/Figures/Energy2M.eps>
<work_palette/Figures/Time2M.eps> [50] <work_palette/Figures/EDP2M.eps>
<work_palette/Figures/AR2M.eps> <work_palette/Figures/Miss2M.eps> [51] [52])
(./work_palette/results2.tex) (./work_palette/conclusion1.tex)) [53]
(./work_cashier/work_cashier.tex
CHAPTER\  7.

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[54] <work_cashier/Cashier_RemappingFigure.eps> [55] [56] [57] [58] [59]
[60] <work_cashier/MSM_Energy_2M.eps> <work_cashier/MSM_Time_2M.eps>
Overfull \hbox (5.7795pt too wide) in paragraph at lines 124--126
 [][] 

Overfull \hbox (5.7795pt too wide) in paragraph at lines 124--126
 [] 
[61] [62]) [63] (./work_master/work_master.tex
CHAPTER\  8.
(./work_master/intro.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[64] [65]) (./work_master/background.tex
<work_master/Figures/BlockDiagram.eps> [66]) (./work_master/method.tex [67]
[68] [69] <work_master/Figures/RCEdesign.eps> [70] [71])
(./work_master/energysavingalgo.tex [72] [73])
(./work_master/hardware_implementation.tex [74] [75])
(./work_master/experimentalmethodology.tex [76] [77] [78]
<work_master/Figures/C2MB4_Energy.eps> <work_master/Figures/C2MB4_WIPC.eps>
[79] [80]) (./work_master/results.tex [81]
<work_master/Figures/C4MB8_Energy.eps> <work_master/Figures/C4MB8_WIPC.eps>
[82] [83]) (./work_master/results2.tex [84]) (./work_master/conclusion.tex
[85])) [86] (./work_manager/work_manager.tex
CHAPTER\  9.
(./work_manager/q_intro.tex
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[87]) (./work_manager/q_methods.tex [88]
<work_manager/Figures/FlowDiagram1.eps> [89] [90]
<work_manager/Figures/RCEdiagram.eps> [91] [92])
(./work_manager/q_energysavingalgorithm.tex [93] [94])
(./work_manager/q_implementation.tex [95])
(./work_manager/q_experimentalplatform.tex [96])
(./work_manager/q_energymodel.tex <work_manager/Figures/C2MB4_Energy.eps>
<work_manager/Figures/C2MB4_AR.eps> <work_manager/Figures/C2MB4_WIPC.eps>
[97] [98]) (./work_manager/q_results.tex [99] [100])
(./work_manager/q_background.tex)) [101] (./work_simulation/work_simulation.tex

CHAPTER\  10.

Package hyperref Warning: Difference (2) between bookmark levels is greater 
(hyperref)                than one, level fixed on input line 4.

<work_simulation/simulation_BlockDiagramMain.eps>
Overfull \hbox (20.46898pt too wide) in paragraph at lines 10--11
 [][] 

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[102] [103] [104] [105] [106] [107] <work_simulation/CPIValueFinal.eps>
<work_simulation/CPIErrorFinal.eps>
Overfull \hbox (27.4011pt too wide) in paragraph at lines 75--77
 [] 

Overfull \hbox (29.23297pt too wide) in paragraph at lines 75--77
 [][] 
[108] [109]) [110] (./work_common/work_publications.tex
CHAPTER\  11.

LaTeX Warning: Citation `MitZha13_Cashier' in file `work_common/work_publicatio
ns' undefined on input line 15.


LaTeX Warning: Citation `Mit2013_DesignContest' in file `work_common/work_publi
cations' undefined on input line 16.


LaTeX Warning: Citation `MitZha12_Simulation' in file `work_common/work_publica
tions' undefined on input line 17.


LaTeX Warning: Citation `MitZha12_EnCache' in file `work_common/work_publicatio
ns' undefined on input line 18.


LaTeX Warning: Citation `mittal_simplex' in file `work_common/work_publications
' undefined on input line 19.


LaTeX Warning: Citation `mittal_fpga' in file `work_common/work_publications' u
ndefined on input line 20.


LaTeX Warning: Citation `mittal_sysgen' in file `work_common/work_publications'
 undefined on input line 21.


LaTeX Warning: Citation `gupta_guaranteed' in file `work_common/work_publicatio
ns' undefined on input line 22.


LaTeX Warning: Citation `GupMit08_MIMO' in file `work_common/work_publications'
 undefined on input line 23.


LaTeX Warning: Citation `MitGup08_BioinQA' in file `work_common/work_publicatio
ns' undefined on input line 24.


LaTeX Warning: Citation `gupta_eureqa' in file `work_common/work_publications' 
undefined on input line 25.


LaTeX Warning: Citation `mittal_caffet' in file `work_common/work_publications'
 undefined on input line 26.

No file work_common/work_publications.bbl.
)
Overfull \vbox (7.05666pt too high) has occurred while \output is active
[111] (./SparshMittal_PhD_Thesis.bbl
Overfull \hbox (9.0pt too wide) in paragraph at lines 1--1
 []   [] 

Overfull \vbox (7.05666pt too high) has occurred while \output is active
[112] [113] [114] [115] [116] [117] [118] [119]
Underfull \hbox (badness 4673) in paragraph at lines 497--501
[]\OT1/cmr/m/n/10.95 M. Monchiero et al.  De-sign space ex-plo-ration for mul-t
i-core ar-chi-tec-tures: a
[120] [121] [122] [123] [124] [125]) [126] (./SparshMittal_PhD_Thesis.aux
(./work_common/titlepage.aux) (./work_common/dedication.aux)
(./work_common/acknowl.aux) (./work_common/abstract.aux)
(./work_common/introduction.aux) (./work_common/contributions.aux)
(./work_common/relatedwork.aux) (./work_esto/work_esto.aux)
(./work_encache/work_encache.aux) (./work_palette/work_palette.aux)
(./work_cashier/work_cashier.aux) (./work_master/work_master.aux)
(./work_manager/work_manager.aux) (./work_simulation/work_simulation.aux)
(./work_common/work_publications.aux))

LaTeX Warning: There were undefined references.

 )
(see the transcript file for additional information)
Output written on SparshMittal_PhD_Thesis.dvi (138 pages, 611056 bytes).
Transcript written on SparshMittal_PhD_Thesis.log.
dvips -t letter -Ppdf -G0 -j0 SparshMittal_PhD_Thesis -o SparshMittal_PhD_Thesis.ps
ps2pdf -dEmbedAllFonts=true -dSubsetFonts=true -dEPSCrop=true -dPDFSETTINGS=/prepress SparshMittal_PhD_Thesis.ps SparshMittal_PhD_Thesis.pdf
acroread SparshMittal_PhD_Thesis.pdf


==> work_manager/q_abstract.tex <==
\begin{abstract}


Last level caches (LLCs) contribute significantly to processor power consumption. Saving LLC energy in multicore QoS systems is especially challenging, since aggressive energy saving techniques may lead to failure in providing QoS. We present MANAGER, a \underline{m}ulticore shared c\underline{a}che e\underline{n}ergy s\underline{a}vin\underline{g} techniqu\underline{e} for quality-of-se\underline{r}vice systems. Using dynamic profiling, MANAGER periodically predicts cache access activity for different configurations. Then, cache is partitioned among running programs to fulfill the QoS requirement while saving memory subsystem (LLC+ DRAM) energy. Out-of-order simulations performed using dual-core workloads from SPEC2006 suite show that for 4MB LLC, MANAGER saves 13.5\% memory subsystem energy, over  a statically, equally-partitioned baseline cache.





\end{abstract}


% Due to recent trends in chip-architecture and CMOS scaling, shared last level caches (LLCs) contribute significantly to processor power consumption. Saving cache energy in multicore QoS systems is especially challenging, since an aggressive energy saving approach may lead to failure in providing QoS. We present MANAGER, a \underline{m}ulticore shared c\underline{a}che e\underline{n}ergy s\underline{a}vin\underline{g} techniqu\underline{e} for quality-of-se\underline{r}vice systems. MANAGER saves leakage energy in shared LLC while providing QoS to one of the running program in best-effort manner. MANAGER partitions cache among running programs such that the target program achieves QoS and memory subsystem (cache+ DRAM) energy is saved. Using dynamic profiling, MANAGER periodically predicts cache access activity for different configurations and reconfigures the cache to a suitable configuration. Out-of-order simulations have been performed using benchmarks from SPEC2006 suite. The results show that for a dual-core configuration with 4MB LLC, the percentage saving in memory subsystem energy, over a  statically, equally-partitioned baseline cache is 14.2\%.

%managing the leakage energy consumption of last level caches (LLCs) has become an important research issue. Achieving In several application scenarios, QoS needs to be ensured for a running program in multicore system. However, existing leakage energy saving techniques work to aggressively save energy and hence may fail to provide QoS. 


% 
% Shared last level caches (LLCs) contribute significantly to processor power consumption. Saving cache energy in multicore QoS systems is especially challenging, since an aggressive energy saving approach may lead to failure in providing QoS. We present MANAGER, a \underline{m}ulticore shared c\underline{a}che e\underline{n}ergy s\underline{a}vin\underline{g} techniqu\underline{e} for quality-of-se\underline{r}vice systems. Using dynamic profiling, MANAGER periodically predicts cache access activity for different configurations. Then, cache is partitioned among running programs to fulfill the QoS requirement while saving memory subsystem (cache+ DRAM) energy. Results from out-of-order simulations performed using benchmarks from SPEC2006 suite show that for a dual-core system with 4MB LLC, MANAGER saves 12.2\% memory subsystem energy, compared to a statically, equally-partitioned baseline cache

==> work_master/abstract.tex <==
\begin{abstract}
With increasing number of on-chip cores and CMOS scaling, the size of last level
caches (LLCs) is on rise and hence, managing their leakage energy consumption has
become vital for continuing to scale performance.  In multicore systems, the locality of memory access
stream is significantly reduced due to multiplexing of access streams from different
running programs and hence, leakage energy saving techniques such as decay cache, which rely on 
memory access locality, do not save large amount of energy. The
techniques based on way level allocation provide very coarse granularity and the techniques based on offline profiling become infeasible to use for large number of cores. 

We present MASTER, a \underline{m}ulticore c\underline{a}che energy
\underline{s}aving \underline{te}chnique using dynamic cache
\underline{r}econfiguration. MASTER uses online profiling to predict energy
consumption of running programs at multiple LLC sizes. Using these estimates,
 suitable cache quotas are allocated to different programs using cache
coloring scheme and the unused LLC space is turned off to save energy. Even for 4
core systems, the implementation overhead of MASTER is only 0.8\% of L2 size. 

We evaluate MASTER using out-of-order simulations with multiprogrammed workloads
from SPEC2006 and compare it with conventional cache leakage energy saving
techniques. The results show that MASTER gives highest saving in  energy and
does not harm performance or cause unfairness. For 2 and 4-core simulations,
the average savings in memory subsystem (which includes LLC and main memory)
energy  over shared baseline LLC are 15\% and 11\%, respectively. Also,
the average values of weighted speedup and fair speedup are close to one ($\ge$0.98).
\end{abstract}




==> work_palette/abstract1.tex <==
\begin{abstract}
With each CMOS technology generation, leakage energy has been increasing at an exponential rate. Since modern processors employ large last level caches (LLCs), their leakage energy consumption has become an important concern in modern chip design.  For addressing this, several techniques have been proposed. However, most of these techniques require offline profiling and hence, cannot be used in real-life systems which run trillions of instructions of arbitrary applications. In this paper, we propose Palette, a technique for saving cache leakage energy using cache coloring. Palette uses a small hardware component called reconfigurable cache emulator, to estimate performance and energy consumption of multiple cache configurations and then selects the configuration with least energy consumption.  Simulations performed with SPEC2006 benchmarks show the superiority of Palette over existing cache energy saving technique. With a 2MB baseline cache, the average saving in memory sub-system energy and EDP are 31.7\% and 29.5\%, respectively.     


\end {abstract}


